Dotted Version Vectors: Logical Clocks for Optimistic Replication

In cloud computing environments, a large number of users access data stored in highly available storage systems. To provide good performance to geographically disperse users and allow operation even in the presence of failures or network partitions, these systems often rely on optimistic replication solutions that guarantee only eventual consistency. In this scenario, it is important to be able to accurately and efficiently identify updates executed concurrently. In this paper, first we review, and expose problems with current approaches to causality tracking in optimistic replication: these either lose information about causality or do not scale, as they require replicas to maintain information that grows linearly with the number of clients or updates. Then, we propose a novel solution that fully captures causality while being very concise in that it maintains information that grows linearly only with the number of servers that register updates for a given data element, bounded by the degree of replication.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusions}

In this paper we have introduced \emph{dotted version vectors}, a novel
solution for tracking causal dependencies among update events. The base idea
of our solution is to efficiently encode the causal history of an update
performed by some client, as a version vector that encodes the causal
history of the previously observed state and a single event identifier
assigned in the server that receives the update.

\emph{Dotted version vectors} allow to accurately track causality among
updates executed by multiple clients using information that is only linear
with the number of servers that register these updates, bounded by the
degree of replication. When compared with previously proposed safe solutions
that require information linear with the number of clients, our solution is
much more efficient, as the number of clients tends to be several orders of
magnitude larger than the number of servers that register updates for a
given data element.


As an evidence that dotted version vectors can be easily used in current
cloud storage systems, we have modified the Riak key-value store to
integrate our solution. Besides the definition of dotted version vectors,
approximately 100 lines of code had to be modified. 

In the future, we intend to study how the underlying idea of dotted version
vectors can be applied to other mechanisms to track causality, such as
extending Interval Tree Clocks \cite{Almeida:2008:ITC:1496310.1496330} in
order to better handle membership changes in the set of replica nodes. 


==> related.tex <==
\section{Related Work}\label{sec:related}

Version tracking solutions as used in cloud storage systems are rooted
on Lamport' seminal work on the definition and role of causality in 
distributed systems~\cite{Lamport78}. This work was  
the foundation for subsequent advances in causality's basic 
mechanisms and theory, including the introduction of version vectors~\cite{PPRSWWCEKK83} for
tracking causality among replicas in a distributed storage system and vector clocks~\cite{Fidge88,Mattern89} for
 tracking causality of events in a distributed systems.


Most of this initial work dealt with a fixed, mostly small, number of 
participants. Later, several systems introduced mechanisms for the dynamic creation
and retirement of vector entries to be used when a server enters and leaves the system. While some techniques required 
the communication with several other servers~\cite{Golding92aweak-consistency}, others required 
communication with a single server~\cite{Petersen97}. Interval Tree Clocks~\cite{Almeida:2008:ITC:1496310.1496330}
are able to track causality in a dynamic, descentralized scenario where entites can be autonomously created
and retired. Other systems, such as Dynamo~\cite{conf/sosp/DeCandiaHJKLPSVV07}, use unsafe techniques to 
remove entries that are expected not to be necessary based on time.

Even with these mechanisms, tracking causality through version vectors or vector clocks 
requires a space linear with the number of entities in the system, posing scalability 
problems for system with a large number of elements~\cite{Charron91}. This problem
is experienced in practice, for example, in cloud computing storage systems, as discussed
in Section~\ref{sec:systems}.

Besides the safe techniques previously mentioned to remove entries that are no longer needed, several other
directions have been tackled to address this problem.

The Roam system~\cite{Ratner98} runs a consensus protocol to decrease, in
all servers, the value of all entries of the version vector by a constant
value. The system only keeps the entries that are larger than zero.  The
\emph{dependency sequences} \cite{PS97} mechanism assumes a scenario where
dynamic, weakly-connected sets of entities (mobile hosts) communicate
through designated proxy entities chosen from a stable, well-connected
(mobile service stations). The mechanism maintains information about the
causal predecessors of each event. It needs to take periodic global
snapshots to prune discardable causality-tracking metadata.

In Depot~\cite{mahajan10depot}, the version vector associated with each
update only includes the entries that have changed since the previous update
in the same node. However, each node still needs to maintain version vectors
that include entries for all clients and servers. In a similar scenario, the
same approach could be used as a complement to our solution. 

Other storage systems explore the fact that they manage a large number of objects to 
maintain less information for each object. In Microsoft's WinFS~\cite{MalTer05}, a base
version vector for all objects is maintained for the file system, and each object maintains only the 
difference for the base in a concise version vector. In Cimbiosys~\cite{Cimbiosys}, the authors
 suggest the use of the same technique in a peer-to-peer system.
These systems, as they maintains only one entry per server, cannot 
generate two concurrent version vectors for tagging concurrent updates
submitted to the same server from 
different clients, as discussed in Section~\ref{sec:systems}.

Another direction is to use unsafe space-folding approaches that can reduce the storage and
communication overhead at the expense of less accuracy of the causality
relation captured by these mechanisms.
Although devised as an alternative not to version vectors but to vector
clocks, \emph{plausible clocks}~\cite{TA99} propose techniques for 
condensing event counting from multiple replicas over the same 
vector entry. The resulting order does not contradict the causal 
precedence relation but because counters are effectively shared between 
processes, some concurrent events will be perceived as causally related. In fact, 
the previously mentioned Lamport clocks~\cite{Lamport78}, are a notable example of plausible clocks.

Another approach trading off less accuracy of causality-tracking for
better scalability is the \emph{hash history} mechanism~\cite{KWK03}. 
It provides a directed graph not of update operations, but of version 
hashes over the state of each replica.
Although independent of the number of replicas in the system, 
the storage overhead grows linearly with the number of updates. In order to 
minimize this problem, it truncates the histories, pruning the oldest 
hashes based on loosely synchronized clocks. Use of hashes, however, 
can only guarantee statistical correctness, and pruning may cause 
incorrect perception of concurrency.




